Vector Projection Network for Few-shot Slot Tagging in Natural Language Understanding

Few-shot slot tagging becomes appealing for rapid domain transfer and adaptation, motivated by the tremendous development of conversational dialogue systems. In this paper, we propose a vector projection network for few-shot slot tagging, which exploits projections of contextual word embeddings on each target label vector as word-label similarities. Essentially, this approach is equivalent to a normalized linear model with an adaptive bias. The contrastive experiment demonstrates that our proposed vector projection based similarity metric can significantly surpass other variants. Specifically, in the five-shot setting on benchmarks SNIPS and NER, our method outperforms the strongest few-shot learning baseline by $6.30$ and $13.79$ points on F$_1$ score, respectively. Our code will be released at https://github.com/sz128/few_shot_slot_tagging_and_NER.

==> tables/1shot_snips.tex <==
 \begin{table*}[htbp]
    \small
    \centering
\begin{tabular}{ccccccccc}
    \hline
    %\multirow{2}{*}{Model} & \multicolumn{7}{c}{1-shot Slot Tagging} & \\ %& \multicolumn{4}{c}{1-shot NER} & \\
    %\cline{2-8} %\cline{10-13}
    \textbf{Model} & \textbf{We} & \textbf{Mu} & \textbf{Pl} & \textbf{Bo} & \textbf{Se} & \textbf{Re} & \textbf{Cr} & \textbf{Avg.} \\ %& News & Wiki & Social & Mixed & Avg. \\
    \hline
    SimBERT & 36.10 & 37.08 & 35.11 & 68.09 & 41.61 & 42.82 & 23.91 & 40.67 \\
    TransferBERT & 55.82 & 38.01 & 45.65 & 31.63 & 21.96 & 41.79 & 38.53 & 39.06 \\
    L-WPZ+CDT+PWE & 71.23	& 47.38	& 59.57	& 81.98	& 69.83	& 66.52	& 62.84	& 65.62 \\
    L-TapNet+CDT+PWE & 71.53	& {60.56}	& 66.27	& \textbf{84.54}	& 76.27	& 70.79	& 62.89	& 70.41 \\
    \hline
    L-TapNet+CDT+VP & 71.65 & \textbf{61.73} & 63.97 & 83.34 & 74.00 & 71.91 & 71.02 & 71.09  \\
    ProtoNet+CDT+VP & \textbf{73.56} & 58.40 & \textbf{68.93} & 82.32 & \textbf{79.69} & \textbf{73.40} & \textbf{70.25} & \textbf{72.37} \\
    ProtoNet+CDT+VPB & 72.65 & 57.35 & 68.72 & 81.92 & 74.68 & 72.48 & 70.04 & 71.12 \\
    \hline
\end{tabular}
    \caption{F$_1$ scores on 1-shot slot tagging of SNIPS dataset.} 
    \label{tab:1shot_snips}
\end{table*}

==> tables/5shot_snips.tex <==
 \begin{table*}[htbp]
    \small
    \centering
\begin{tabular}{ccccccccc}
    \hline
    %\multirow{2}{*}{Model} & \multicolumn{7}{c}{1-shot Slot Tagging} & \\ %& \multicolumn{4}{c}{1-shot NER} & \\
    %\cline{2-8} %\cline{10-13}
    \textbf{Model} & \textbf{We} & \textbf{Mu} & \textbf{Pl} & \textbf{Bo} & \textbf{Se} & \textbf{Re} & \textbf{Cr} & \textbf{Avg.} \\ %& News & Wiki & Social & Mixed & Avg. \\
    \hline
    SimBERT & 53.46 & 54.13 & 42.81 & 75.54 & 57.10 & 55.30 & 32.38 & 52.96 \\
    TransferBERT & 59.41 & 42.00 & 46.07 & 20.74 & 28.20 & 67.75 & 58.61 & 46.11 \\
    L-WPZ+CDT+PWE & 74.68 & 56.73 & 52.20 & 78.79 & 80.61 & 69.59 & 67.46 & 68.58 \\
    L-TapNet+CDT+PWE & 71.64 & 67.16 & 75.88 & 84.38 & 82.58 & 70.05 & 73.41 & 75.01 \\
    \hline
    L-TapNet+CDT+VP & 78.25 & {67.79} & 70.66 & 86.17 & 75.80 & 78.51 & 75.93 & 76.16  \\
    ProtoNet+CDT+VP & {79.88} & {67.77} & {78.08} & {87.68} & \textbf{86.59} & {79.95} & {75.61} & {79.37} \\
    ProtoNet+CDT+VPB & \textbf{82.91} & \textbf{69.23} & \textbf{80.85} & \textbf{90.69} & 86.38 & \textbf{81.20} & \textbf{76.75} & \textbf{81.14} \\
    \hline
\end{tabular}
    \caption{F$_1$ scores on 5-shot slot tagging of SNIPS dataset.} 
    \label{tab:5shot_snips}
\end{table*}
